Quantitative Global Memory

We show that recent approaches of static analysis based on quantitative typing systems can be extended to programming languages with global state. More precisely, we define a call-by-value language equipped with operations to access a global memory, together with a semantic model based on a (tight) multi-type system that captures exact measures of time and space related to evaluation of programs. We show that the type system is quantitatively sound and complete with respect to the original operational semantics of the language.

==> proofs/comp-notabs-implies-negabs.tex <==
\begin{proof}
    By induction over $\Phi$:
    \begin{itemize}
        \item Case $\Phi$ ends with rule (\ruleAx), (\ruleApp), (\ruleAppPOne), or (\ruleAppPTwo), $\neg\isabs{t}$ holds by definition.
        \item Case $\Phi$ ends with rule (\ruleLam), (\ruleMany), or (\ruleLamP), $\tau \not\in \nott{\tabs}$. Therefore, these cases do not apply.
    \end{itemize}
\end{proof}

==> proofs/lem-comp-reduction-expansion.tex <==
\begin{proof} \mbox{}
    \begin{enumerate}
        \item \input{proofs/lem-comp-subj-red}
        \item \input{proofs/lem-comp-subj-exp}
    \end{enumerate}    
\end{proof}

==> proofs/lem-comp-soundness-completeness.tex <==
\begin{proof} \mbox{}
    \begin{enumerate}
        \item \input{proofs/thm-gs-soundness}
        \item \input{proofs/lem-comp-completeness}
    \end{enumerate}
\end{proof}

==> proofs/lem-comp-subs-antisubs.tex <==
\begin{proof} \mbox{}
    \begin{enumerate}
        \item \input{proofs/lem-comp-subs}
        \item \input{proofs/lem-comp-antisubs}
    \end{enumerate}
\end{proof}

==> proofs/lem-reduction-expansion.tex <==
\begin{proof} \mbox{}
    \begin{enumerate}
        \item \input{proofs/lem-subj-red}
        \item \input{proofs/lem-subj-exp}
    \end{enumerate}
\end{proof}

==> proofs/lem-soundness-completeness.tex <==
\begin{proof}\mbox{}
    \begin{enumerate}
        \item \input{proofs/thm-soundness}
        \item \input{proofs/thm-completeness}
    \end{enumerate}
\end{proof}

==> proofs/lem-subs-antisubs.tex <==
\begin{proof} \mbox{}
    \begin{enumerate}
        \item \input{proofs/lem-subs}
        \item \input{proofs/lem-antisubs}
    \end{enumerate}
\end{proof}



==> proofs/lem-tight-nfs.tex <==
\begin{proof}
    By simultaneous induction over the following claims: \begin{enumerate}
        \item \label{lem:tight-nfs:1} If $\Phi \tr \seqi{\Gam}{t}{\stype \ra \tneutral \tim \stype'}{(0,0,s)}$, then $t \in \neutral$.
        \item \label{lem:tight-nfs:2} If $\Phi \tr \seqi{\Gam}{t}{\stype \ra \tightt \tim \stype'}{(0,0,s)}$, then $t \in \normal$.
    \end{enumerate}
    \begin{enumerate}
        \item By induction over $\Phi$: \begin{itemize}
            \item Case $\Phi$ ends with ($\ruleApp$). Then $t = v u$, $\Phi_u \tr \seqi{\Gam_u}{u}{\stype \ra \M \tim \stype'}{(0,0,r_u)}$, $\Phi_v \tr \seqi{\Gam_v}{v}{\M \ra \stype' \ra \del \tim \stype''}{(0,0,0,r_v)}$, such that $\Gam_t = \Gam_u + \Gam_v$ tight, $\del = \tneutral$, and $r = r_u + r_v$. But, by~\cref{lem:tight-zero}, $\stype \ra \M \tim \stype'$ tight. Absurd, since $\M \not\in \tightt$. Therefore, this case does not apply.
            \item Case $\Phi$ ends with ($\ruleAppPOne$). This case does not apply since $\tneutral \not= $.
            \item Case $\Phi$ ends with ($\ruleAppPTwo$). This case does not apply since $\tneutral \not= $.
            \item Case $\Phi$ ends with ($\ruleGet$). This case does not apply since $g > 0$.
            \item Case $\Phi$ ends with ($\ruleSet$). This case does not apply since $s > 0$.
        \end{itemize}
        \item By induction over $\Phi$: \begin{itemize}
            \item Case $\Phi$ ends with ($\ruleApp$). Then $t = v u$, $\Phi_u \tr \seqi{\Gam_u}{u}{\stype \ra \M \tim \stype'}{(0,0,0,r_u)}$, $\Phi_v \tr \seqi{\Gam_v}{v}{\M \ra \stype' \ra \del \tim \stype''}{(0,0,r_v)}$, such that $\Gam_t = \Gam_u + \Gam_v$ tight, $\del = $, and $r = r_u + r_v$. But, by~\cref{lem:tight-zero}, $\stype \ra \M \tim \stype'$ tight. Absurd, since $\M \not\in \tightt$. Therefore, this case does not apply.
            \item Case $\Phi$ ends with ($\ruleAppPOne$). Then $t = v u$, $\Phi_u \tr \seqi{\Gam_u}{u}{\stype \ra \tneutral \tim \stype'}{(0,0,r_u)}$, $\Phi_v \tr \seqi{\Gam_v}{v}{\tightv}{(0,0,0,r_v)}$, such that $\Gam_t = \Gam_u + \Gam_v$ tight and $r = r_u + r_v$. By the \ih (\cref{lem:tight-nfs:2}), we have $u \in \neutral$. Therefore, $v u \in \neutral$.
            \item Case $\Phi$ ends with ($\ruleAppPTwo$). Then $t = v u$, $\Phi_u \tr \seqi{\Gam_u}{u}{\stype \ra \tightt \tim \stype'}{(0,0,r_u)}$, $\Phi_v \tr \seqi{\Gam_v}{v}{\tvar}{(0,0,r_v)}$, such that $\Gam_t = \Gam_u + \Gam_v$ tight and $r = r_u + r_v$. By the \ih(\cref{lem:tight-nfs:3}), we have $u \in \normal$. By~\cref{prop:tightvalue}, we have $v = x$. Therefore, $x u \in \neutral$.
            \item Case $\Phi$ ends with ($\ruleGet$). This case does not apply since $g > 0$.
            \item Case $\Phi$ ends with ($\ruleSet$). This case does not apply since $s > 0$.
        \end{itemize}
        \item This case is subsumed by the two previous cases.
    \end{enumerate}
\end{proof}


==> proofs/lem-zero-size.tex <==
By induction on $\Phi$: 
\begin{itemize}
    \item Case $\Phi$ ends with ($\ruleApp$). This case does not apply, since it does not conclude with a tight type.
    \item Case $\Phi$ ends with ($\ruleAppPOne$). Then $t = v u$ and $\Phi \tr \seqi{\Gam' + \Del}{v u}{\tneutral}{(0,0,r'+r''+1)}$. Therefore, $\Phi_u \tr \seqi{\Gam'}{u}{\tneutral}{(0,0,r)}$ and $\Phi_V \tr \seqi{\Del}{V}{\tightv}{(0,0,0,r')}$ are tight. By the \ih, we have $r' = \size{u}$. By~\cref{prop:tightvaluezero}, we have $r'' = 0$. Therefore, $r = r'+r''+1 = \size{u} + 0 + 1 = \size{u} + \size{V} + 1 = \size{v u}$.
    \item Case $\Phi$ ends with ($\ruleAppPTwo$). Then $t = v u$ and $\Phi \tr \seqi{\Gam' + \Del}{v u}{\tneutral}{(0,0,0,r'+r''+1)}$. Therefore, $\Phi_u \tr \seqi{\Gam'}{u}{\tightt}{(0,0,r)}$ and $\Phi_V \tr \seqi{\Del}{v}{\tvar}{(0,0,0,r')}$ are tight. By the \ih, we have $r' = \size{u}$. By~\cref{prop:tightvaluezero}, we have $r'' = 0$. Therefore, $r = r'+r''+1 = \size{u} + 0 + 1 = \size{u} + \size{v} + 1 = \size{v u}$.
    \item Case $\Phi$ ends with ($\ruleGet$). This case does not apply, since it does not conclude with a tight type.
    \item Case $\Phi$ ends with ($\ruleSet$). This case does not apply, since it does not conclude with a tight type.
\end{itemize}


==> proofs/lem-zero-tight-store.tex <==
\begin{proof}
    By induction over $M \in \normal$: \begin{itemize}
        \item Case $M \in \ne$, then we have to consider two additional cases: \begin{itemize}
            \item Case $t = x u$. Then $N \in \normal$ and $\Phi_M$ must end with ($\ruleAppPOne$) or ($\ruleAppPTwo$), since $N$ should have a tight type by~\cref{lem:tight-zero}. In either case, we can conclude by applying the \ih to the type derivation for $N$, which will tell us that $\sig = \sig'$.
            \item Case $t = (\lam x.p)u$. Then $N \in \neutral \subseteq \normal$ and $\Phi_t$ must end with ($\ruleAppPOne$), since $N$ should have a tight type by~\cref{lem:tight-zero} and $\lam x.p$ cannot have type $\tvar$, by~\cref{prop:tightvalue}. But, then we can conclude by applying the \ih to the type derivation for $N$, which will tell us that $\sig = \sig'$.
        \end{itemize}
    \end{itemize}
\end{proof}
